Carbon-Aware Optimal Power Flow

To facilitate effective decarbonization of the electric power sector, this paper introduces the generic Carbon-aware Optimal Power Flow (C-OPF) method for power system decision-making that considers demand-side carbon accounting and emission management. Built upon the classic optimal power flow (OPF) model, the C-OPF method incorporates carbon emission flow equations and constraints, as well as carbon-related objectives, to jointly optimize power flow and carbon flow. In particular, this paper establishes the feasibility and solution uniqueness of the carbon emission flow equations, and proposes modeling and linearization techniques to address the issues of undetermined power flow directions and bilinear terms in the C-OPF model. Additionally, two novel carbon emission models, together with the carbon accounting schemes, for energy storage systems are developed and integrated into the C-OPF model. Numerical simulations demonstrate the characteristics and effectiveness of the C-OPF method, in comparison with OPF solutions.

==> Biography.tex <==

 

\vskip -4pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{xin}}]{Xin Chen} is an Assistant Professor in the Department of Electrical and Computer Engineering at Texas A\&M University (TAMU). Dr. Chen directs the Smart Power, Energy and Decision-making (SPEED) Lab at TAMU. His research lies in the intersection of control, machine/reinforcement learning, and optimization for smart sustainable power and energy systems. He received the Ph.D. degree in electrical engineering from Harvard University, the master’s degree in electrical engineering and two bachelor’s degrees in engineering and economics from Tsinghua University. He was a Postdoctoral Associate affiliated with MIT Energy Initiative at Massachusetts Institute of Technology. He is a recipient of the IEEE PES Outstanding Doctoral Dissertation Award, IEEE Transactions on Smart Grid Top-5 Outstanding Papers, and multiple best paper awards at IEEE control and power conferences.  
\end{IEEEbiography}

\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{andy}}]{Andy Sun} is is the Iberdrola-Avangrid Professor in Electric Power Systems in the Sloan School of Management at the Massachusetts Institute of Technology (MIT). He received his PhD degree in Operations Research from MIT and was a postdoctoral fellow in the Mathematical Sciences division of the IBM T. J. Watson Research Center at Yorktown Heights, NY. He was a faculty member in the School of Industrial and Systems Engineering at Georgia Institute of Technology before joining MIT. Dr. Sun's research focuses on optimization and computation for large-scale electric power system control, operations, and planning, market design for power grid decarbonization, and electrification of transportation. His research on robust operation of power grids has been influential in improving reliability unit commitment in ISO/RTO markets.  
\end{IEEEbiography}

\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wenbo}}]{Wenbo Shi} is the Founder/CEO of Singularity Energy, a startup that offers advanced carbon and clean energy management software and data solutions for utilities, grid operators,
corporations and technology providers to accurately measure emissions and optimize their decision-making for grid decarbonization. Singularity is proud to partner with organizations such as Southern Company, MISO, Eversource Energy, Enersponse, Sense, and Measurable.Before founding Singularity, Wenbo was a postdoctoral researcher at Harvard University. He received his Ph.D. from University of California, Los Angeles in 2015.
\end{IEEEbiography}


\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{lina}}]{Na Li}
 is a Winokur Family Professor of Electrical Engineering and Applied Mathematics at Harvard University.  She received her Bachelor's degree in Mathematics from Zhejiang University in 2007 and Ph.D. degree in Control and Dynamical systems from California Institute of Technology in 2013. She was a postdoctoral associate at the Massachusetts Institute of Technology 2013-2014.  She has held a variety of short-term visiting appointments including the Simons Institute for the Theory of Computing, MIT, Google Brain, and MERL. Her research lies in the control, learning, and optimization of networked systems, including theory development, algorithm design, and applications to real-world cyber-physical societal system. 
\end{IEEEbiography}


 
